Finding $r$-II sibling stars in the Milky Way with the Greedy Optimistic Clustering algorithm

$R$-process enhanced stars with [Eu/Fe]$\geq+0.7$ (so-called $r$-II stars) are believed to have formed in an extremely neutron-rich environment in which a rare astrophysical event (e.g., a neutron star merger) occurred. This scenario is supported by the existence of an ultra-faint dwarf galaxy, Reticulum~II, where most of the stars are highly enhanced in $r$-process elements. In this scenario, some small fraction of dwarf galaxies around the Milky Way were $r$ enhanced. When each $r$-enhanced dwarf galaxy accreted to the Milky Way, it deposited many $r$-II stars in the Galactic halo with similar orbital actions. To search for the remnants of the $r$-enhanced systems, we analyzed the distribution of the orbital actions of $N=161$ $r$-II stars in the Solar neighborhood by using the Gaia EDR3 data. Since the observational uncertainty is not negligible, we applied a newly-developed {\it greedy optimistic clustering method} to the orbital actions of our sample stars. We found six clusters of $r$-II stars that have similar orbits and chemistry, one of which is a new discovery. Given the apparent phase-mixed orbits of the member stars, we interpret that these clusters are good candidates for remnants of completely disrupted $r$-enhanced dwarf galaxies that merged with the ancient Milky Way.

==> tab2_all_original.tex <==
\startlongtable
\begin{deluxetable*}{l l c cccc }
\tablecaption{Basic properties of the member stars of the clusters 
\label{table:members_all_info}}
%\rotate %%Kohei
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{$k$} &
\colhead{R18} &
\colhead{Name} &
\colhead{([Fe/H],[Eu/H],[Eu/Fe])} &
\colhead{$(J_r,J_z,J_\phi)$} &
\colhead{$E$} &
\colhead{$\varpi/\sigma_\varpi$} \\
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{dex} &
\colhead{$\kpc \kms$} &
\colhead{$10^5 \;(\mathrm{\kms})^2$} &
\colhead{} 
%&
%\colhead{Star name} &
%\colhead{List} %\\
%\colhead{$P_\text{gap-forming}$ $^\mathrm{(a)}$} &
%\colhead{$N_\text{gap-forming}$ $^\mathrm{(b)}$} &
%\colhead{List of $k$ for gap-forming orbits$^\mathrm{(c)}$} %\\
%%%{} & {(GC id)} & {(Probability of forming} & {(Number of} \\
%%%{} & {} & {a gap in the GD-1 stream)} & {gap-forming orbits)} 
}
\startdata
{1} & {} & {HE 1523-0901} & {$(-2.95, -1.14, +1.81)$} & {$(148, 366, +1219)$} & {$-1.558$} & {$16.626$}\\
{1} & {} & {RAVE J203843.2-002333} & {$(-2.91, -1.27, +1.64)$} & {$(99, 269, +1400)$} & {$-1.559$} & {$11.179$}\\
{1} & {} & {2MASS J09544277+5246414} & {$(-2.99, -1.71, +1.28)$} & {$(216, 462, +1319)$} & {$-1.482$} & {$26.830$}\\
{1} & {} & {2MASS J17225742-7123000} & {$(-2.42, -1.35, +1.07)$} & {$(143, 396, +1212)$} & {$-1.553$} & {$18.841$}\\
{1} & {} & {2MASS J20050670-3057445} & {$(-3.03, -2.09, +0.94)$} & {$(378, 80, +1208)$} & {$-1.565$} & {$20.871$}\\
{1} & {} & {HE 1044-2509} & {$(-2.89, -1.95, +0.94)$} & {$(87, 410, +1237)$} & {$-1.564$} & {$11.977$}\\
{1} & {} & {J14592981-3852558} & {$(-2.40, -1.47, +0.93)$} & {$(10, 146, +993)$} & {$-1.790$} & {$13.810$}\\
{1} & {} & {BPS CS 22896-154} & {$(-2.69, -1.83, +0.86)$} & {$(10, 83, +1076)$} & {$-1.793$} & {$17.928$}\\
{1} & {} & {2MASS J01555066-6400155} & {$(-2.71, -1.91, +0.80)$} & {$(70, 171, +1218)$} & {$-1.662$} & {$17.600$}\\
\hline
{2} & {} & {SMSS J175046.30-425506.9} & {$(-2.17, -0.42, +1.75)$} & {$(966, 55, +117)$} & {$-1.606$} & {$2.798$}\\
{2} & {D} & {HD 222925} & {$(-1.47, -0.14, +1.33)$} & {$(1052, 84, +273)$} & {$-1.520$} & {$189.056$}\\
{2} & {} & {RAVE J071142.5-343237} & {$(-1.96, -0.66, +1.30)$} & {$(774, 3, +228)$} & {$-1.709$} & {$43.802$}\\
{2} & {} & {2MASS J18024226-4404426} & {$(-1.55, -0.50, +1.05)$} & {$(796, 150, +154)$} & {$-1.642$} & {$16.274$}\\
{2} & {} & {J11404944-1615396} & {$(-1.67, -0.79, +0.88)$} & {$(925, 109, +57)$} & {$-1.620$} & {$16.332$}\\
{2} & {} & {J07352232-4425010} & {$(-1.58, -0.79, +0.79)$} & {$(1041, 27, +46)$} & {$-1.604$} & {$184.629$}\\
{2} & {D} & {HD 20} & {$(-1.60, -0.87, +0.73)$} & {$(1115, 9, -99)$} & {$-1.572$} & {$92.637$}\\
{2} & {D} & {2MASS J01530024-3417360} & {$(-1.50, -0.79, +0.71)$} & {$(972, 5, +37)$} & {$-1.657$} & {$231.958$}\\
{2} & {} & {HD 3567} & {$(-1.33, -0.63, +0.70)$} & {$(835, 24, +105)$} & {$-1.692$} & {$412.636$}\\
\hline
{3} & {} & {2MASS J00512646-1053170} & {$(-2.38, -1.17, +1.21)$} & {$(420, 219, -810)$} & {$-1.600$} & {$189.026$}\\
{3} & {A} & {HE 0430-4901} & {$(-2.72, -1.56, +1.16)$} & {$(427, 121, -719)$} & {$-1.669$} & {$27.471$}\\
{3} & {} & {2MASS J22562536-0719562} & {$(-2.26, -1.16, +1.10)$} & {$(371, 121, -636)$} & {$-1.726$} & {$11.873$}\\
{3} & {} & {SDSS J173025.57+414334.7} & {$(-2.85, -1.77, +1.08)$} & {$(706, 45, -788)$} & {$-1.557$} & {$39.280$}\\
{3} & {F} & {HE 2224+0143} & {$(-2.58, -1.53, +1.05)$} & {$(338, 51, -592)$} & {$-1.805$} & {$16.152$}\\
{3} & {} & {J03422816-6500355} & {$(-2.16, -1.11, +1.05)$} & {$(365, 14, -688)$} & {$-1.778$} & {$98.567$}\\
{3} & {A} & {BPS CS 22958-052} & {$(-2.42, -1.42, +1.00)$} & {$(435, 21, -895)$} & {$-1.660$} & {$68.063$}\\
{3} & {} & {SDSS J004305.27+194859.20} & {$(-2.25, -1.27, +0.98)$} & {$(534, 36, -652)$} & {$-1.679$} & {$35.415$}\\
{3} & {} & {BPS CS 22875-029} & {$(-2.69, -1.77, +0.92)$} & {$(389, 352, -655)$} & {$-1.618$} & {$11.905$}\\
{3} & {F} & {HD 115444} & {$(-2.96, -2.11, +0.85)$} & {$(601, 25, -603)$} & {$-1.667$} & {$67.006$}\\
{3} & {} & {J01425445-0904162} & {$(-1.73, -0.90, +0.83)$} & {$(372, 37, -891)$} & {$-1.684$} & {$47.161$}\\
{3} & {} & {G206-23} & {$(-1.79, -0.98, +0.81)$} & {$(688, 361, -695)$} & {$-1.476$} & {$305.366$}\\
{3} & {A} & {HD 221170} & {$(-2.18, -1.38, +0.80)$} & {$(379, 16, -962)$} & {$-1.669$} & {$79.320$}\\
{3} & {} & {HE 0420+0123a} & {$(-3.03, -2.24, +0.79)$} & {$(367, 232, -622)$} & {$-1.680$} & {$41.097$}\\
{3} & {} & {RAVE J015656.3-140211} & {$(-2.08, -1.32, +0.76)$} & {$(704, 203, -621)$} & {$-1.543$} & {$14.705$}\\
{3} & {} & {BPS CS 22877-015} & {$(-2.00, -1.28, +0.72)$} & {$(399, 12, -531)$} & {$-1.819$} & {$103.131$}\\
{3} & {} & {J12044314-2911051} & {$(-2.35, -1.64, +0.71)$} & {$(489, 202, -829)$} & {$-1.574$} & {$31.947$}\\
{3} & {A} & {2MASS J15271353-2336177} & {$(-2.15, -1.45, +0.70)$} & {$(357, 28, -659)$} & {$-1.778$} & {$46.190$}\\
\hline
{4} & {C} & {2MASS J21064294-6828266} & {$(-2.76, -1.44, +1.32)$} & {$(62, 314, -901)$} & {$-1.716$} & {$40.082$}\\
{4} & {} & {J05383296-5904280} & {$(-2.53, -1.25, +1.28)$} & {$(198, 257, -890)$} & {$-1.670$} & {$80.688$}\\
{4} & {C} & {BPS CS 22945-017} & {$(-2.73, -1.60, +1.13)$} & {$(150, 200, -1029)$} & {$-1.673$} & {$35.846$}\\
{4} & {} & {2MASS J18174532-3353235} & {$(-1.67, -0.68, +0.99)$} & {$(126, 146, -871)$} & {$-1.769$} & {$3.870$}\\
{4} & {} & {RAVE J133748.9-082617} & {$(-2.62, -1.69, +0.93)$} & {$(125, 281, -795)$} & {$-1.731$} & {$5.305$}\\
{4} & {C} & {2MASS J15582962-1224344} & {$(-2.54, -1.65, +0.89)$} & {$(18, 222, -951)$} & {$-1.763$} & {$22.353$}\\
{4} & {} & {2MASS J17163340-7009028} & {$(-2.39, -1.50, +0.89)$} & {$(23, 207, -919)$} & {$-1.780$} & {$10.026$}\\
{4} & {} & {BPS CS 30306-132} & {$(-2.42, -1.57, +0.85)$} & {$(244, 157, -926)$} & {$-1.678$} & {$21.118$}\\
{4} & {} & {J20435776-4408037} & {$(-1.85, -1.07, +0.78)$} & {$(65, 138, -852)$} & {$-1.818$} & {$12.669$}\\
{4} & {} & {2MASS J21095804-0945400} & {$(-2.73, -1.96, +0.77)$} & {$(95, 143, -864)$} & {$-1.792$} & {$9.632$}\\
{4} & {} & {2MASS J19215077-4452545} & {$(-2.56, -1.82, +0.74)$} & {$(106, 176, -887)$} & {$-1.758$} & {$4.410$}\\
{4} & {} & {2MASS J17435113-5359333} & {$(-2.24, -1.51, +0.73)$} & {$(105, 144, -754)$} & {$-1.829$} & {$25.874$}\\
\hline
{5} & {} & {2MASS J02462013-1518419} & {$(-2.71, -1.26, +1.45)$} & {$(1087, 281, +796)$} & {$-1.358$} & {$21.971$}\\
{5} & {G} & {BPS CS 22953-003} & {$(-2.84, -1.79, +1.05)$} & {$(951, 388, +768)$} & {$-1.383$} & {$18.803$}\\
{5} & {G} & {HE 2327-5642} & {$(-2.78, -1.80, +0.98)$} & {$(877, 531, +749)$} & {$-1.380$} & {$12.640$}\\
{5} & {} & {SMSS J183647.89-274333.1} & {$(-2.48, -1.66, +0.82)$} & {$(927, 380, +773)$} & {$-1.390$} & {$3.254$}\\
{5} & {} & {HE 0300-0751} & {$(-2.27, -1.50, +0.77)$} & {$(930, 190, +777)$} & {$-1.435$} & {$0.990$}\\
\hline
{6} & {} & {2MASS J05241392-0336543} & {$(-2.50, -1.00, +1.50)$} & {$(103, 133, -2497)$} & {$-1.352$} & {$4.395$}\\
{6} & {} & {2MASS J07150266-0154092} & {$(-2.60, -1.72, +0.88)$} & {$(31, 2, -2512)$} & {$-1.403$} & {$30.915$}\\
\hline
{7} & {} & {SMSS J062609.83-590503.2} & {$(-2.77, -1.71, +1.06)$} & {$(914, 176, -2835)$} & {$-1.133$} & {$13.632$}\\
{7} & {} & {HE 2244-1503} & {$(-2.88, -1.93, +0.95)$} & {$(1029, 237, -2662)$} & {$-1.126$} & {$6.843$}\\
\hline
{8} & {} & {J07202253-3358518} & {$(-1.60, -0.16, +1.44)$} & {$(3527, 3318, +52)$} & {$-0.813$} & {$69.734$}\\
{8} & {} & {Gaia DR2 2233912206910720000} & {$(-1.72, -0.61, +1.11)$} & {$(3510, 3462, +274)$} & {$-0.796$} & {$25.346$}\\
\hline
{9} & {B} & {SDSS J235718.91-005247.8} & {$(-3.36, -1.44, +1.92)$} & {$(139, 755, +927)$} & {$-1.525$} & {$43.974$}\\
{9} & {B} & {BPS CS 31082-001} & {$(-2.90, -1.27, +1.63)$} & {$(85, 1019, +855)$} & {$-1.496$} & {$17.304$}\\
{9} & {} & {SDSS J092157.27+503404.7} & {$(-2.65, -1.42, +1.23)$} & {$(118, 791, +834)$} & {$-1.549$} & {$27.046$}\\
{9} & {B} & {SMSS J051008.62-372019.8} & {$(-3.20, -2.25, +0.95)$} & {$(90, 695, +829)$} & {$-1.588$} & {$83.448$}\\
{9} & {} & {BPS CS 22888-047} & {$(-2.54, -1.68, +0.86)$} & {$(21, 739, +862)$} & {$-1.595$} & {$4.769$}\\
{9} & {} & {SMSS J195931.70-643529.3} & {$(-2.58, -1.84, +0.74)$} & {$(219, 1238, +665)$} & {$-1.444$} & {$8.568$}\\
\hline
{10} & {} & {HE 2301-4024} & {$(-2.11, -1.13, +0.98)$} & {$(794, 1019, +1181)$} & {$-1.249$} & {$2.984$}\\
{10} & {} & {BPS CS 29491-069} & {$(-2.55, -1.59, +0.96)$} & {$(889, 1314, +1276)$} & {$-1.180$} & {$22.426$}\\
{10} & {} & {2MASS J19324858-5908019} & {$(-1.93, -1.03, +0.90)$} & {$(895, 1252, +1184)$} & {$-1.196$} & {$4.210$}\\
{10} & {} & {HE 1131+0141} & {$(-2.48, -1.61, +0.87)$} & {$(934, 1175, +1188)$} & {$-1.199$} & {$2.078$}\\
\hline
{11} & {} & {G15-13} & {$(-1.47, -0.62, +0.85)$} & {$(1038, 355, +1757)$} & {$-1.217$} & {$639.873$}\\
{11} & {} & {G115-58} & {$(-1.30, -0.55, +0.75)$} & {$(835, 420, +1756)$} & {$-1.248$} & {$116.967$}\\
\hline
{12} & {} & {2MASS J22182082-3827554} & {$(-2.57, -1.47, +1.10)$} & {$(269, 1227, -1000)$} & {$-1.367$} & {$24.310$}\\
{12} & {} & {2MASS J03270229+0132322} & {$(-2.39, -1.32, +1.07)$} & {$(243, 1336, -1361)$} & {$-1.294$} & {$64.065$}\\
\hline
{13} & {} & {2MASS J14534137+0040467} & {$(-3.09, -1.29, +1.80)$} & {$(541, 791, -166)$} & {$-1.552$} & {$4.740$}\\
{13} & {} & {2MASS J13052137-1137220} & {$(-2.07, -0.98, +1.09)$} & {$(478, 719, +84)$} & {$-1.634$} & {$6.495$}\\
{13} & {} & {HE 1127-1143} & {$(-2.73, -1.65, +1.08)$} & {$(363, 861, +110)$} & {$-1.642$} & {$1.829$}\\
{13} & {} & {SMSS J221448.33-453949.9} & {$(-2.56, -1.62, +0.94)$} & {$(344, 1012, +90)$} & {$-1.587$} & {$0.148$}\\
{13} & {} & {2MASS J12091322-1415313} & {$(-2.11, -1.30, +0.81)$} & {$(434, 727, +160)$} & {$-1.632$} & {$16.765$}\\
{13} & {} & {RAVE J192632.8-584657} & {$(-2.49, -1.73, +0.76)$} & {$(538, 736, +5)$} & {$-1.614$} & {$5.545$}\\
\hline
{14} & {} & {2MASS J15213995-3538094} & {$(-2.79, -0.56, +2.23)$} & {$(922, 366, -2107)$} & {$-1.194$} & {$36.738$}\\
{14} & {} & {2MASS J01553180-4919420} & {$(-3.01, -2.29, +0.72)$} & {$(1016, 142, -1773)$} & {$-1.253$} & {$58.543$}\\
\hline
{15} & {} & {BPS CS 22892-052} & {$(-3.10, -1.46, +1.64)$} & {$(679, 358, -335)$} & {$-1.576$} & {$6.801$}\\
{15} & {H} & {2MASS J21091825-1310062} & {$(-2.40, -1.15, +1.25)$} & {$(488, 136, -88)$} & {$-1.849$} & {$28.003$}\\
{15} & {E} & {BPS CS 22945-058} & {$(-2.71, -1.58, +1.13)$} & {$(624, 72, -214)$} & {$-1.753$} & {$28.693$}\\
{15} & {} & {2MASS J14543792+0830379} & {$(-2.31, -1.21, +1.10)$} & {$(391, 176, -157)$} & {$-1.866$} & {$17.143$}\\
{15} & {} & {SMSS J181505.16-385514.9} & {$(-3.29, -2.33, +0.96)$} & {$(452, 53, -136)$} & {$-1.916$} & {$3.207$}\\
{15} & {} & {J00041581-5815524} & {$(-2.32, -1.37, +0.95)$} & {$(529, 341, +74)$} & {$-1.729$} & {$14.929$}\\
{15} & {} & {2MASS J19014952-4844359} & {$(-1.87, -0.94, +0.93)$} & {$(453, 43, -125)$} & {$-1.930$} & {$19.104$}\\
{15} & {E} & {BD +17 3248} & {$(-2.06, -1.15, +0.91)$} & {$(572, 45, -110)$} & {$-1.838$} & {$95.470$}\\
{15} & {F} & {BPS CS 29529-054} & {$(-2.75, -1.85, +0.90)$} & {$(596, 59, -274)$} & {$-1.756$} & {$59.902$}\\
{15} & {E} & {2MASS J00405260-5122491} & {$(-2.11, -1.25, +0.86)$} & {$(582, 35, -166)$} & {$-1.817$} & {$423.879$}\\
{15} & {} & {G210-33} & {$(-1.08, -0.31, +0.77)$} & {$(738, 200, -396)$} & {$-1.576$} & {$364.784$}\\
{15} & {H} & {2MASS J19232518-5833410} & {$(-2.08, -1.32, +0.76)$} & {$(558, 98, -186)$} & {$-1.788$} & {$29.542$}\\
{15} & {} & {J18050641-4907579} & {$(-2.58, -1.85, +0.73)$} & {$(325, 48, -246)$} & {$-1.977$} & {$13.794$}\\
{15} & {} & {RAVE J000738.2-034551} & {$(-2.09, -1.36, +0.73)$} & {$(629, 95, -260)$} & {$-1.722$} & {$8.238$}\\
{15} & {} & {BPS BS 17569-049} & {$(-2.88, -2.16, +0.72)$} & {$(521, 345, -36)$} & {$-1.743$} & {$6.694$}\\
{15} & {} & {J23342332-2748003} & {$(-2.35, -1.64, +0.71)$} & {$(481, 226, -151)$} & {$-1.775$} & {$13.352$}\\
{15} & {} & {2MASS J13494713-7423395} & {$(-2.85, -2.15, +0.70)$} & {$(363, 263, -146)$} & {$-1.845$} & {$28.769$}\\
{15} & {} & {SMSS J182601.24-332358.3} & {$(-2.83, -2.13, +0.70)$} & {$(496, 113, -218)$} & {$-1.806$} & {$7.387$}\\
\hline
{16} & {} & {HE 1219-0312} & {$(-2.92, -1.54, +1.38)$} & {$(361, 292, +539)$} & {$-1.687$} & {$2.126$}\\
{16} & {} & {2MASS J20093393-3410273} & {$(-1.99, -0.67, +1.32)$} & {$(258, 231, +641)$} & {$-1.735$} & {$8.035$}\\
{16} & {} & {2MASS J15383085-1804242} & {$(-2.09, -0.82, +1.27)$} & {$(321, 150, +454)$} & {$-1.806$} & {$66.989$}\\
{16} & {} & {J07103110-7121522} & {$(-1.47, -0.42, +1.05)$} & {$(551, 17, +573)$} & {$-1.706$} & {$146.784$}\\
{16} & {} & {2MASS J15211026-0607566} & {$(-2.00, -1.07, +0.93)$} & {$(293, 270, +545)$} & {$-1.734$} & {$30.961$}\\
{16} & {} & {J20000364-3301351} & {$(-1.89, -0.99, +0.90)$} & {$(189, 198, +445)$} & {$-1.880$} & {$14.214$}\\
{16} & {} & {RAVE J194550.6-392631} & {$(-2.79, -1.89, +0.90)$} & {$(81, 116, +522)$} & {$-1.984$} & {$12.934$}\\
{16} & {} & {BPS BS 16543-097} & {$(-2.48, -1.63, +0.85)$} & {$(369, 93, +554)$} & {$-1.774$} & {$29.222$}\\
{16} & {} & {RAVE J093730.5-062655} & {$(-1.86, -1.01, +0.85)$} & {$(565, 247, +608)$} & {$-1.586$} & {$18.012$}\\
{16} & {} & {BPS CS 22882-001} & {$(-2.62, -1.81, +0.81)$} & {$(487, 415, +462)$} & {$-1.605$} & {$3.864$}\\
{16} & {} & {RAVE J130524.5-393126} & {$(-2.11, -1.35, +0.76)$} & {$(327, 72, +496)$} & {$-1.835$} & {$26.463$}\\
{16} & {} & {LP877-23} & {$(-1.46, -0.71, +0.75)$} & {$(261, 438, +410)$} & {$-1.725$} & {$385.595$}\\
{16} & {B} & {HE 1430+0053} & {$(-3.03, -2.31, +0.72)$} & {$(356, 237, +530)$} & {$-1.719$} & {$16.215$}\\
\hline
{17} & {} & {Gaia DR2 6412626111276193920} & {$(-2.04, -0.27, +1.77)$} & {$(29, 1161, -393)$} & {$-1.598$} & {$0.658$}\\
{17} & {} & {2MASS J00101758-1735387} & {$(-2.41, -1.06, +1.35)$} & {$(0, 1245, -569)$} & {$-1.539$} & {$74.434$}\\
{17} & {} & {2MASS J23362202-5607498} & {$(-2.06, -0.92, +1.14)$} & {$(100, 1078, -369)$} & {$-1.601$} & {$10.327$}\\
{17} & {} & {LAMOST J112456.61+453531.1} & {$(-1.27, -0.17, +1.10)$} & {$(387, 1096, -344)$} & {$-1.494$} & {$5.019$}\\
\hline
{18} & {} & {2MASS J03073894-0502491} & {$(-2.22, -0.95, +1.27)$} & {$(376, 238, -1874)$} & {$-1.373$} & {$7.300$}\\
{18} & {} & {HE 0432-0923} & {$(-3.19, -1.94, +1.25)$} & {$(328, 242, -1852)$} & {$-1.388$} & {$4.483$}\\
{18} & {} & {2MASS J02165716-7547064} & {$(-2.50, -1.38, +1.12)$} & {$(407, 250, -1942)$} & {$-1.349$} & {$18.601$}\\
\hline
{19} & {} & {SMSS J183128.71-341018.4} & {$(-1.83, -0.58, +1.25)$} & {$(54, 216, -249)$} & {$-2.100$} & {$6.064$}\\
{19} & {} & {2MASS J19161821-5544454} & {$(-2.35, -1.27, +1.08)$} & {$(101, 216, -345)$} & {$-1.988$} & {$10.641$}\\
{19} & {} & {SMSS J183225.29-334938.4} & {$(-1.74, -0.66, +1.08)$} & {$(183, 311, -262)$} & {$-1.898$} & {$1.034$}\\
{19} & {} & {SMSS J175738.37-454823.5} & {$(-2.46, -1.44, +1.02)$} & {$(38, 306, -198)$} & {$-2.079$} & {$5.578$}\\
{19} & {} & {2MASS J21224590-4641030} & {$(-2.96, -2.06, +0.90)$} & {$(139, 579, -460)$} & {$-1.725$} & {$17.135$}\\
{19} & {} & {2MASS J18294359-4924253} & {$(-1.22, -0.33, +0.89)$} & {$(61, 151, -234)$} & {$-2.162$} & {$12.451$}\\
{19} & {} & {J20411424-4654315} & {$(-2.30, -1.42, +0.88)$} & {$(302, 225, -204)$} & {$-1.880$} & {$11.797$}\\
\hline
{20} & {} & {SMSS J155430.57-263904.8} & {$(-2.61, -1.47, +1.14)$} & {$(1297, 444, -1027)$} & {$-1.245$} & {$6.169$}\\
{20} & {} & {2MASS J00524174-0902235} & {$(-1.46, -0.52, +0.94)$} & {$(1283, 379, -940)$} & {$-1.269$} & {$29.465$}\\
{20} & {} & {HE 0240-0807} & {$(-2.68, -1.95, +0.73)$} & {$(1328, 367, -1020)$} & {$-1.260$} & {$0.323$}\\
{20} & {} & {RAVE J091858.9-231151} & {$(-2.05, -1.34, +0.71)$} & {$(1324, 179, -1080)$} & {$-1.273$} & {$15.284$}\\
\hline
{21} & {} & {2MASS J14325334-4125494} & {$(-2.79, -1.18, +1.61)$} & {$(2151, 227, -1013)$} & {$-1.116$} & {$52.981$}\\
{21} & {} & {Gaia DR2 1508756353921427328} & {$(-1.93, -1.16, +0.77)$} & {$(2175, 204, -1091)$} & {$-1.114$} & {$23.097$}\\
\hline
{22} & {} & {2MASS J12170829+0415146} & {$(-2.22, -1.12, +1.10)$} & {$(1486, 1239, +401)$} & {$-1.188$} & {$0.577$}\\
{22} & {} & {BPS CS 30315-029} & {$(-3.33, -2.61, +0.72)$} & {$(1509, 1267, +324)$} & {$-1.190$} & {$4.335$}\\
\hline
{23} & {} & {HE 1226-1149} & {$(-2.91, -1.36, +1.55)$} & {$(156, 645, -1760)$} & {$-1.369$} & {$5.527$}\\
{23} & {} & {J22372037-4741375} & {$(-2.97, -2.13, +0.84)$} & {$(180, 521, -1553)$} & {$-1.428$} & {$13.029$}\\
{23} & {} & {J10401894-4106124} & {$(-1.55, -0.73, +0.82)$} & {$(164, 619, -1751)$} & {$-1.374$} & {$42.487$}\\
\hline
{24} & {} & {BPS CS 29497-004} & {$(-2.85, -1.18, +1.67)$} & {$(365, 239, -1406)$} & {$-1.471$} & {$12.522$}\\
{24} & {} & {BPS CS 31078-018} & {$(-2.84, -1.61, +1.23)$} & {$(275, 25, -1215)$} & {$-1.634$} & {$44.957$}\\
{24} & {} & {J22190836-2333467} & {$(-2.54, -1.67, +0.87)$} & {$(106, 108, -1167)$} & {$-1.690$} & {$22.914$}\\
{24} & {C} & {BPS CS 22943-132} & {$(-2.67, -1.81, +0.86)$} & {$(62, 221, -1374)$} & {$-1.598$} & {$141.707$}\\
{24} & {} & {BPS CS 22886-012} & {$(-2.61, -1.76, +0.85)$} & {$(106, 25, -1165)$} & {$-1.738$} & {$19.888$}\\
{24} & {} & {J10191573-1924464} & {$(-1.11, -0.36, +0.75)$} & {$(126, 42, -1368)$} & {$-1.646$} & {$23.505$}\\
{24} & {} & {J06195001-5312114} & {$(-2.06, -1.33, +0.73)$} & {$(72, 258, -1299)$} & {$-1.602$} & {$149.166$}\\
{24} & {} & {J14354680-1124122} & {$(-1.10, -0.38, +0.72)$} & {$(16, 10, -1556)$} & {$-1.656$} & {$76.502$}\\
{24} & {} & {RAVE J183623.2-642812} & {$(-2.50, -1.78, +0.72)$} & {$(15, 41, -1294)$} & {$-1.730$} & {$27.378$}\\
{24} & {} & {HD 120559} & {$(-1.31, -0.60, +0.71)$} & {$(52, 15, -1493)$} & {$-1.656$} & {$136.429$}\\
{24} & {} & {2MASS J18295183-4503394} & {$(-2.48, -1.78, +0.70)$} & {$(10, 20, -1358)$} & {$-1.722$} & {$46.753$}\\
{24} & {} & {BD-10 3742 } & {$(-1.96, -1.26, +0.70)$} & {$(81, 46, -1288)$} & {$-1.694$} & {$32.606$}\\
{24} & {} & {J06320130-2026538} & {$(-1.56, -0.86, +0.70)$} & {$(137, 65, -1308)$} & {$-1.647$} & {$155.373$}\\
{24} & {} & {RAVE J115941.7-382043} & {$(-0.94, -0.24, +0.70)$} & {$(46, 7, -1512)$} & {$-1.658$} & {$87.671$}\\
\hline
{25} & {} & {G166-37} & {$(-1.18, -0.32, +0.86)$} & {$(5072, 2134, -601)$} & {$-0.735$} & {$357.603$}\\
{25} & {} & {HE 2252-4225} & {$(-2.63, -1.82, +0.81)$} & {$(5051, 2365, -133)$} & {$-0.747$} & {$2.050$}\\
\hline
{26} & {} & {RAVE J040618.2-030525} & {$(-1.34, -0.17, +1.17)$} & {$(1801, 130, -18)$} & {$-1.272$} & {$58.391$}\\
{26} & {} & {LAMOST J110901+075441} & {$(-3.17, -2.23, +0.94)$} & {$(1727, 196, -366)$} & {$-1.289$} & {$9.180$}\\
{26} & {} & {Gaia DR2 3602288924850161792 } & {$(-1.89, -1.09, +0.80)$} & {$(1566, 158, -339)$} & {$-1.321$} & {$27.652$}\\
{26} & {} & {CD -45 3283} & {$(-0.99, -0.21, +0.78)$} & {$(1577, 178, -119)$} & {$-1.321$} & {$153.969$}\\
\hline
{27} & {} & {Gaia DR2 4248140165233284352} & {$(-1.82, -1.12, +0.70)$} & {$(1485, 1831, +579)$} & {$-1.102$} & {$12.291$}\\
\hline
{28} & {} & {G14-39} & {$(-1.88, -1.10, +0.78)$} & {$(727, 1284, -585)$} & {$-1.310$} & {$501.058$}\\
\hline
{29} & {} & {SMSS J024858.41-684306.4} & {$(-3.71, -2.71, +1.00)$} & {$(6120, 342, -2857)$} & {$-0.662$} & {$20.514$}\\
\hline
{30} & {} & {SMSS J063447.15-622355.0} & {$(-3.41, -2.52, +0.89)$} & {$(8014, 274, -3751)$} & {$-0.560$} & {$8.100$\cite{Jacobson_et_al__2015}}\\
\hline
\enddata
%\tablecomments{
%(a) Something I want to say! 
%}
\end{deluxetable*}
